Revealing Domain-Spatiality Patterns for Configuration Tuning: Domain Knowledge Meets Fitness Landscapes

Configuration tuning for better performance is crucial in quality assurance. Yet, there has long been a mystery on tuners' effectiveness, due to the black-box nature of configurable systems. Prior efforts predominantly adopt static domain analysis (e.g., static taint analysis), which often lacks generalizability, or dynamic data analysis (e.g., benchmarking performance analysis), limiting explainability. In this work, we embrace Fitness Landscape Analysis (FLA) as a bridge between domain knowledge and difficulty of the tuning. We propose Domland, a two-pronged methodology that synergizes the spatial information obtained from FLA and domain-driven analysis to systematically capture the hidden characteristics of configuration tuning cases, explaining how and why a tuner might succeed or fail. This helps to better interpret and contextualize the behavior of tuners and inform tuner design. To evaluate Domland, we conduct a case study of nine software systems and 93 workloads, from which we reveal several key findings: (1) configuration landscapes are inherently system-specific, with no single domain factor (e.g., system area, programming language, or resource intensity) consistently shaping their structure; (2) the core options (e.g., pic-struct of x264), which control the main functional flows, exert a stronger influence on landscape ruggedness (i.e. the difficulty of tuning) compared to resource options (e.g., cpu-independent of x264); (3) Workload effects on landscape structure are not uniformly tied to type or scale. Both contribute to landscape variations, but their impact is system-dependent.

==> paper_sections/metrics.tex <==

\section{Introduction}
\label{section:introduction}


\subsection{Landscape Metrics}
\label{subsection: Landscape Metrics}

\subsubsection{Fitness Distance Correlation (FDC)}
FDC is a widely used metric for evaluating the relationship between the fitness (e.g., runtime and throughput) of solutions (i.e., configurations) and their distance to the global optimum in a given landscape~\cite{jones1995fitness}. It helps to characterize the global structure of the fitness landscape and evaluate the ease or difficulty of navigating toward the global optimum. Formally, FDC is calculated as:

\begin{equation}
\varrho(f, d)=\frac{1}{\sigma_f \sigma_d} \frac{1}{s}\sum_{i=1}^s\left(f_i-\bar{f}\right)\left(d_i-\bar{d}\right),
\end{equation}
where $s$ is the number of solutions considered in FDC. Within such a solutions set, $d_i$ denotes the distance of $i$th solution to the nearest global optimum. $\bar{f}$ ($\bar{d}$) and $\sigma_f$ ($\sigma_d$) are the mean and standard deviation of fitness (and distance). 

%For minimization problems, their can be roughly categorized into three classes based on FDC ($\varrho$) values~\cite{jones1995fitness}:

% \begin{itemize}
%     \item\textbf{\textit{Straightforward}} ($\varrho$ $\geq$ 0.15), in which fitness tends to decrease with distance from the global optimum, guiding the search towards the optimal solution.
%     \item \textbf{\textit{Difficult}} ($\mathcal{-}0.15 \textless \varrho \textless 0.15$), in which there is a trivial correlation between fitness and distance from global optima.
%     \item \textbf{\textit{Misleading}} ($\varrho \leq \mathcal{-} 0.15$), in which fitness tends to increase with distance from the global optimum, misleading the search.
% \end{itemize}

%Following this classification, FDC provides valuable insights into the structural properties of software systems' performance landscapes. By quantifying the relationship between configuration quality and proximity to the optimal solution, FDC helps practitioners in understanding the properties hidden inside the system. 


%Particularly, in this study, the only exception is the \textsc{h2} system, which is a maximization problem focused on maximizing throughput. To ensure consistency in calculating the FDC value, we invert the performance values for the \textsc{h2} system. This adjustment allows for a standardized interpretation of FDC across all studied systems.

%Hence, FDC is an effective measure for evaluating the global landscape structure, evolvability, and potential deception with optimization problems.





\subsubsection{Local optima} Local optima capture the underlying local structural properties of a problem's landscape. Formally, a configuration \textbf{\textit{c}}$^{\ell}$ is considered as a local optima if $f(\textbf{\textit{c}}^{\ell})$ is better than $f(\textbf{\textit{c}})$, $\forall \textbf{\textit{c}} \in \mathcal{N}\left(\textbf{\textit{c}}^{\ell}\right)$, where $\mathcal{N}\left(\textbf{\textit{c}}^{\ell}\right)$ is the neighborhood of \textbf{\textit{c}}$^{\ell}$. Two key aspects are considered when analyzing local optima: (1) the number of local optima; and (2) the quality of local optima.


(1) \textit{The number of local optima} reflects landscape multimodality, indicating the presence of multiple high-performing regions and complexity of the problem. To quantify this, we define $\ell_p$ as the proportion of local optima among all sampled configurations:
\begin{equation}
    \ell_p = \frac{|\mathcal{L}|}{\mathcal{|S|}},
\end{equation}
where $\mathcal{L}$ and $\mathcal{S}$ denote the sets of local optima and all sampled configurations, respectively.

(2) \textit{The quality of local optima}---particularly their relative performance compared to the global optima---indicates the prominence of local peaks and the susceptibility of the landscape to trapping suboptimal solutions. For minimization problems, we define the relative quality of local optima as:
    
\begin{equation}
\ell_q = \frac{\frac{1}{|\mathcal{S}|} \sum\limits_{\textbf{\textit{c}} \in S} f(\textbf{\textit{c}}) - \frac{1}{|\mathcal{L}|} \sum\limits_{\textbf{\textit{c}}^\ell \in \mathcal{L}} f(\textbf{\textit{c}}^\ell)}
{\frac{1}{|\mathcal{S}|} \sum\limits_{\textbf{\textit{c}} \in \mathcal{S}} f(\textbf{\textit{c}}) - f(\textbf{\textit{c}}^g)},
\end{equation}
where $\textbf{\textit{c}}^g$ represents the global optimum, and $\textbf{\textit{c}}^\ell$ denotes a local optima from $\mathcal{L}$. A higher $\ell_q$ indicates that local optima are of higher quality, being closer to the global optimum, while a lower $\ell_q$ suggests an abundance of low-quality local optima.

% \begin{itemize}
%     \item[1)] \textbf{\textit{The number of local optima}} provides insight into the landscape's multimodality, revealing the extent to which multiple distinct regions of relatively superior performance exist. This multimodality reflects the inherent complexity of the problem and the potential for diverse, competing solutions. To provide a more intuitive measure, we introduce $\ell_p$, which represents the proportion of local optima relative to all sampled configurations in a landscape, as follows:
%     \begin{equation}
%         \ell_p = \frac{|\mathcal{L}|}{\mathcal{|S|}},
%     \end{equation}
%     where $\mathcal{L}$ and $\mathcal{S}$ denote the sets of local optima and all sampled configurations, respectively.
    
%     \item[2)] \textbf{\textit{The quality of local optima}}---particularly their relative performance compared to the global optima---indicates the prominence of local peaks and the susceptibility of the landscape to trapping suboptimal solutions. For minimization problems, we define the relative quality of local optima as:
    
%     \begin{equation}
%     \ell_q = \frac{\frac{1}{|\mathcal{S}|} \sum\limits_{\textbf{\textit{c}} \in S} f(\textbf{\textit{c}}) - \frac{1}{|\mathcal{L}|} \sum\limits_{\textbf{\textit{c}}^\ell \in \mathcal{L}} f(\textbf{\textit{c}}^\ell)}
%     {\frac{1}{|\mathcal{S}|} \sum\limits_{\textbf{\textit{c}} \in \mathcal{S}} f(\textbf{\textit{c}}) - f(\textbf{\textit{c}}^g)},
%     \end{equation}
%     where $\textbf{\textit{c}}^g$ represents the global optimum, and $\textbf{\textit{c}}^\ell$ denotes a local optima from $\mathcal{L}$. A higher $\ell_q$ value indicates that local optima exhibit high overall quality, as their performance is closer to the global optimum. In contrast, a lower $\ell_q$ suggests the presence of many low-quality local optima, making optimization more challenging.
% \end{itemize}




\subsubsection{Basin of attraction}
The basin of attraction of a local optimum \( \textbf{\textit{c}}^\ell \), denoted as \( \mathcal{B}(\textbf{\textit{c}}^\ell) \), is the set of all configurations that converge to \( \textbf{\textit{c}}^\ell \) under a local search process. Formally, it can be defined as:

\begin{equation}
\mathcal{B}(\textbf{\textit{c}}^\ell) = \{ \textbf{\textit{c}} \in \mathcal{C} \mid \text{LocalSearch}(\textbf{\textit{c}}) \to \textbf{\textit{c}}^\ell \}.
\end{equation}


%, providing insights into the structural continuity of the landscape surface
\subsubsection{Autocorrelation}
Autocorrelation quantifies the ruggedness of a fitness landscape by measuring how fitness values change across neighboring configurations. Formally, it is defined as:

\begin{equation}
\label{eq:autocorrelation}
r(d) =\frac{\sum_{i=1}^{N-d}\left(f\left(\textbf{\textit{c}}_i\right)-\bar{f}\right)\left(f\left(\textbf{\textit{c}}_{i+d}\right)-\bar{f}\right)}{\sum_{i=1}^{N-d}\left(f\left(\textbf{\textit{c}}_i\right)-\bar{f}\right)^2},
\end{equation}
where $f(\textbf{\textit{c}}_i)$ is the fitness of $i$th visited configuration $\textbf{\textit{c}}_i$ in the random walk~\cite{tavares2008multidimensional}, $\textbf{\textit{c}}_{i+d}$ is the next visited neighbor at step size $d$, and $N$ is the walk length. A high $r(d)$ indicates a smooth landscape, where similar configurations yield comparable fitness values, while a low autocorrelation suggests a rugged landscape with abrupt fitness variations.




==> tables/2-Ratio-Quality.tex <==

\begin{tabular}{c|cc|c|cc|c|cc|c|cc|c|cc|c|cc|c|cc|c|cc|c|cc}
\toprule
\multirow{2}{*}{\textbf{Workload}} & \multicolumn{2}{c|}{\textbf{Lrzip}}                  & \multicolumn{1}{l|}{\textbf{}} & \multicolumn{2}{c|}{\textbf{Xz}}                     & \multicolumn{1}{l|}{\textbf{}} & \multicolumn{2}{c|}{\textbf{Z3}}                     & \multicolumn{1}{l|}{\textbf{}} & \multicolumn{2}{c|}{\textbf{Dconvert}}               & \multicolumn{1}{l|}{\textbf{}} & \multicolumn{2}{c|}{\textbf{Batlik}}                 & \multicolumn{1}{l|}{\textbf{}} & \multicolumn{2}{c|}{\textbf{Kanzi}}                   & \multicolumn{1}{l|}{\textbf{}} & \multicolumn{2}{c|}{\textbf{X264}}                   & \multicolumn{1}{l|}{\textbf{}} & \multicolumn{2}{c|}{\textbf{H2}}                     & \multicolumn{1}{l|}{\textbf{}} & \multicolumn{2}{c}{\textbf{Jump3r}}                  \\ \cline{2-27} 
                                   & \multicolumn{1}{c|}{\textbf{$\ell_r$}}     & \textbf{$\ell_q$}     & \textbf{}                      & \multicolumn{1}{c|}{\textbf{R}}     & \textbf{Q}     & \textbf{}                      & \multicolumn{1}{c|}{\textbf{R}}     & \textbf{Q}     & \textbf{}                      & \multicolumn{1}{c|}{\textbf{R}}     & \textbf{Q}     & \textbf{}                      & \multicolumn{1}{c|}{\textbf{R}}     & \textbf{Q}     & \textbf{}                      & \multicolumn{1}{c|}{\textbf{R}}     & \textbf{Q}      & \textbf{}                      & \multicolumn{1}{c|}{\textbf{R}}     & \textbf{Q}     & \textbf{}                      & \multicolumn{1}{c|}{\textbf{R}}     & \textbf{Q}     & \textbf{}                      & \multicolumn{1}{c|}{\textbf{R}}     & \textbf{Q}     \\ \midrule
W1                                 & \multicolumn{1}{c|}{0.120}          & 0.972          &                                & \multicolumn{1}{c|}{0.179}          & 0.482          &                                & \multicolumn{1}{c|}{0.015}          & 0.628          &                                & \multicolumn{1}{c|}{0.006}          & 0.787          &                                & \multicolumn{1}{c|}{0.017}          & 0.754          &                                & \multicolumn{1}{c|}{0.086}          & -0.333          &                                & \multicolumn{1}{c|}{0.280}          & 0.049          &                                & \multicolumn{1}{c|}{0.026}          & 0.244          &                                & \multicolumn{1}{c|}{0.041}          & 0.376          \\
W2                                 & \multicolumn{1}{c|}{0.194}          & 0.992          &                                & \multicolumn{1}{c|}{0.426}          & 0.321          &                                & \multicolumn{1}{c|}{0.125}          & 0.784          &                                & \multicolumn{1}{c|}{0.005}          & 0.753          &                                & \multicolumn{1}{c|}{0.009}          & 0.906          &                                & \multicolumn{1}{c|}{0.105}          & -0.234          &                                & \multicolumn{1}{c|}{0.255}          & 0.037          &                                & \multicolumn{1}{c|}{0.025}          & 0.071          &                                & \multicolumn{1}{c|}{0.042}          & 0.534          \\
W3                                 & \multicolumn{1}{c|}{0.099}          & 0.987          &                                & \multicolumn{1}{c|}{0.193}          & 0.420          &                                & \multicolumn{1}{c|}{0.024}          & 0.967          &                                & \multicolumn{1}{c|}{0.026}          & 0.569          &                                & \multicolumn{1}{c|}{0.010}          & 0.788          &                                & \multicolumn{1}{c|}{0.147}          & 0.421           &                                & \multicolumn{1}{c|}{0.270}          & 0.062          &                                & \multicolumn{1}{c|}{0.024}          & 0.232          &                                & \multicolumn{1}{c|}{0.044}          & 0.510          \\
W4                                 & \multicolumn{1}{c|}{0.105}          & 0.945          &                                & \multicolumn{1}{c|}{0.170}          & 0.501          &                                & \multicolumn{1}{c|}{0.016}          & 0.966          &                                & \multicolumn{1}{c|}{0.005}          & 0.739          &                                & \multicolumn{1}{c|}{0.011}          & 0.890          &                                & \multicolumn{1}{c|}{0.084}          & -0.338          &                                & \multicolumn{1}{c|}{0.266}          & 0.048          &                                & \multicolumn{1}{c|}{0.028}          & 0.316          &                                & \multicolumn{1}{c|}{0.048}          & 0.450          \\
W5                                 & \multicolumn{1}{c|}{0.099}          & 0.830          &                                & \multicolumn{1}{c|}{0.172}          & 0.344          &                                & \multicolumn{1}{c|}{0.012}          & 0.992          &                                & \multicolumn{1}{c|}{0.008}          & 0.718          &                                & \multicolumn{1}{c|}{0.011}          & 0.879          &                                & \multicolumn{1}{c|}{0.086}          & -0.247          &                                & \multicolumn{1}{c|}{0.265}          & 0.054          &                                & \multicolumn{1}{c|}{0.030}          & 0.101          &                                & \multicolumn{1}{c|}{0.042}          & 0.396          \\
W6                                 & \multicolumn{1}{c|}{0.099}          & 0.959          &                                & \multicolumn{1}{c|}{0.201}          & 0.327          &                                & \multicolumn{1}{c|}{0.022}          & 0.996          &                                & \multicolumn{1}{c|}{0.018}          & 0.540          &                                & \multicolumn{1}{c|}{0.016}          & 0.826          &                                & \multicolumn{1}{c|}{0.089}          & -0.296          &                                & \multicolumn{1}{c|}{0.393}          & 0.093          &                                & \multicolumn{1}{c|}{0.027}          & 0.060          &                                & \multicolumn{1}{c|}{0.056}          & 0.467          \\
W7                                 & \multicolumn{1}{c|}{0.141}          & 0.904          &                                & \multicolumn{1}{c|}{0.248}          & 0.405          &                                & \multicolumn{1}{c|}{0.057}          & 0.829          &                                & \multicolumn{1}{c|}{0.004}          & 0.610          &                                & \multicolumn{1}{c|}{0.008}          & 0.964          &                                & \multicolumn{1}{c|}{0.092}          & -0.282          &                                & \multicolumn{1}{c|}{0.293}          & 0.111          &                                & \multicolumn{1}{c|}{0.028}          & 0.283          &                                & \multicolumn{1}{c|}{N/A}            & N/A            \\
W8                                 & \multicolumn{1}{c|}{0.089}          & 0.974          &                                & \multicolumn{1}{c|}{0.168}          & 0.412          &                                & \multicolumn{1}{c|}{0.070}          & 0.973          &                                & \multicolumn{1}{c|}{0.009}          & 0.652          &                                & \multicolumn{1}{c|}{0.012}          & 0.857          &                                & \multicolumn{1}{c|}{0.087}          & -0.293          &                                & \multicolumn{1}{c|}{0.383}          & 0.100          &                                & \multicolumn{1}{c|}{0.028}          & 0.376          &                                & \multicolumn{1}{c|}{N/A}            & N/A            \\
W9                                 & \multicolumn{1}{c|}{0.089}          & 0.972          &                                & \multicolumn{1}{c|}{0.187}          & 0.353          &                                & \multicolumn{1}{c|}{0.147}          & 0.938          &                                & \multicolumn{1}{c|}{0.016}          & 0.578          &                                & \multicolumn{1}{c|}{0.022}          & 0.767          &                                & \multicolumn{1}{c|}{0.089}          & 0.266           &                                & \multicolumn{1}{c|}{0.349}          & 0.101          &                                & \multicolumn{1}{c|}{N/A}            & N/A            &                                & \multicolumn{1}{c|}{N/A}            & N/A            \\
W10                                & \multicolumn{1}{c|}{0.115}          & 0.945          &                                & \multicolumn{1}{c|}{0.171}          & 0.419          &                                & \multicolumn{1}{c|}{0.020}          & 0.803          &                                & \multicolumn{1}{c|}{0.033}          & 0.671          &                                & \multicolumn{1}{c|}{0.011}          & 0.900          &                                & \multicolumn{1}{c|}{N/A}            & N/A             &                                & \multicolumn{1}{c|}{N/A}            & N/A            &                                & \multicolumn{1}{c|}{N/A}            & N/A            &                                & \multicolumn{1}{c|}{N/A}            & N/A            \\
W11                                & \multicolumn{1}{c|}{0.120}          & 0.935          &                                & \multicolumn{1}{c|}{0.170}          & 0.424          &                                & \multicolumn{1}{c|}{0.013}          & 0.695          &                                & \multicolumn{1}{c|}{0.020}          & 0.510          &                                & \multicolumn{1}{c|}{0.007}          & 0.964          &                                & \multicolumn{1}{c|}{N/A}            & N/A             &                                & \multicolumn{1}{c|}{N/A}            & N/A            &                                & \multicolumn{1}{c|}{N/A}            & N/A            &                                & \multicolumn{1}{c|}{N/A}            & N/A            \\
W12                                & \multicolumn{1}{c|}{0.105}          & 0.951          &                                & \multicolumn{1}{c|}{0.169}          & 0.437          &                                & \multicolumn{1}{c|}{0.010}          & 0.995          &                                & \multicolumn{1}{c|}{0.019}          & 0.775          &                                & \multicolumn{1}{c|}{N/A}            & N/A            &                                & \multicolumn{1}{c|}{N/A}            & N/A             &                                & \multicolumn{1}{c|}{N/A}            & N/A            &                                & \multicolumn{1}{c|}{N/A}            & N/A            &                                & \multicolumn{1}{c|}{N/A}            & N/A            \\
W13                                & \multicolumn{1}{c|}{0.110}          & 0.980          &                                & \multicolumn{1}{c|}{0.192}          & 0.307          &                                & \multicolumn{1}{c|}{N/A}            & N/A            &                                & \multicolumn{1}{c|}{N/A}            & N/A            &                                & \multicolumn{1}{c|}{N/A}            & N/A            &                                & \multicolumn{1}{c|}{N/A}            & N/A             &                                & \multicolumn{1}{c|}{N/A}            & N/A            &                                & \multicolumn{1}{c|}{N/A}            & N/A            &                                & \multicolumn{1}{c|}{N/A}            & N/A            \\ \midrule
\textbf{Median}                    & \multicolumn{1}{c|}{\textbf{0.105}} & \textbf{0.959} & \textbf{}                      & \multicolumn{1}{c|}{\textbf{0.179}} & \textbf{0.412} & \textbf{}                      & \multicolumn{1}{c|}{\textbf{0.021}} & \textbf{0.952} & \textbf{}                      & \multicolumn{1}{c|}{\textbf{0.012}} & \textbf{0.661} & \textbf{}                      & \multicolumn{1}{c|}{\textbf{0.011}} & \textbf{0.879} & \textbf{}                      & \multicolumn{1}{c|}{\textbf{0.089}} & \textbf{-0.282} & \textbf{}                      & \multicolumn{1}{c|}{\textbf{0.280}} & \textbf{0.062} & \textbf{}                      & \multicolumn{1}{c|}{\textbf{0.028}} & \textbf{0.238} & \textbf{}                      & \multicolumn{1}{c|}{\textbf{0.043}} & \textbf{0.458} \\ \midrule
\textbf{Std}                       & \multicolumn{1}{c|}{\textbf{0.028}} & \textbf{0.043} & \textbf{}                      & \multicolumn{1}{c|}{\textbf{0.070}} & \textbf{0.061} & \textbf{}                      & \multicolumn{1}{c|}{\textbf{0.047}} & \textbf{0.129} & \textbf{}                      & \multicolumn{1}{c|}{\textbf{0.009}} & \textbf{0.096} & \textbf{}                      & \multicolumn{1}{c|}{\textbf{0.004}} & \textbf{0.073} & \textbf{}                      & \multicolumn{1}{c|}{\textbf{0.020}} & \textbf{0.283}  & \textbf{}                      & \multicolumn{1}{c|}{\textbf{0.054}} & \textbf{0.028} & \textbf{}                      & \multicolumn{1}{c|}{\textbf{0.002}} & \textbf{0.119} & \textbf{}                      & \multicolumn{1}{c|}{\textbf{0.006}} & \textbf{0.062} \\ \bottomrule
\end{tabular}


==> tables/subject_systems.tex <==
\begin{tabular}{lllllccc}
\toprule
\textbf{System} & \textbf{Lang.} & \textbf{Domain} & \textbf{Perf.} & \textbf{Version}             & \textbf{\#O} & \textbf{\#C} & \textbf{\#W} \\ \midrule

\textsc{Jump3r}       & Java       & Audio Encoder   & Runtime        & 1.0.4                        & 13           & 4196         & 6            \\
\textsc{Kanzi}         & Java       & File Compressor & Runtime        & 1.9                          & 18           & 4112         & 9            \\
\textsc{Dconvert}   & Java       & Image Scaling   & Runtime        & 1.0.0-$\alpha$7              & 10           & 6764         & 12           \\
\textsc{H2}               & Java       & Database        & Throughput     & 1.4.200                      & 16           & 1954         & 8            \\
\textsc{Batlik}      & Java       & SVG Rasterizer  & Runtime        & 1.14                         & 8            & 1919         & 11           \\ \midrule
\textsc{Xz}               & C/C++      & File Compressor & Runtime        & 5.2.0                        & 12           & 1999         & 13           \\
\textsc{Lrzip}         & C/C++      & File Compressor & Runtime        & 0.651                        & 7            & 190          & 13           \\
\textsc{X264}           & C/C++      & Video Encoder   & Runtime        & baee400…                     & 25           & 3113         & 9            \\
\textsc{Z3}               & C/C++      & SMT Solver      & Runtime        & 4.8.14                       & 12           & 1011         & 12           \\ 

\bottomrule
\end{tabular}
